Causal Discovery in Physical Systems from Videos

Causal discovery is at the core of human cognition. It enables us to reason about the environment and make counterfactual predictions about unseen scenarios that can vastly differ from our previous experiences. We consider the task of causal discovery from videos in an end-to-end fashion without supervision on the ground-truth graph structure. In particular, our goal is to discover the structural dependencies among environmental and object variables: inferring the type and strength of interactions that have a causal effect on the behavior of the dynamical system. Our model consists of (a) a perception module that extracts a semantically meaningful and temporally consistent keypoint representation from images, (b) an inference module for determining the graph distribution induced by the detected keypoints, and (c) a dynamics module that can predict the future by conditioning on the inferred graph. We assume access to different configurations and environmental conditions, i.e., data from unknown interventions on the underlying system; thus, we can hope to discover the correct underlying causal graph without explicit interventions. We evaluate our method in a planar multi-body interaction environment and scenarios involving fabrics of different shapes like shirts and pants. Experiments demonstrate that our model can correctly identify the interactions from a short sequence of images and make long-term future predictions. The causal structure assumed by the model also allows it to make counterfactual predictions and extrapolate to systems of unseen interaction graphs or graphs of various sizes.

==> tabText/future_prediction.tex <==
\begin{table}[t]
\caption{{\bf Quantitative results on future prediction.} In this table, we show our model's performance of future prediction. Our model first observes $100$ frames of the system, infers the discrete and continuous variables on the causal graph, and then predicts multiple steps into the future. Note that we only train our model in environments containing $5$ balls, which automatically generalize to unseen scenarios of different numbers of balls. For clarity, the values in the table are scaled by $10^4$.}
\label{tab:future_pred}
\begin{center}\small

\begin{tabular}{c|cccc}
\toprule
Time & $T + 1$ & $T + 5$ & $T + 10$ & $T + 20$ \\
\midrule
$3$ balls & 3.04 (3.27) & 14.9 (22.8) & 48.0 (66.3) & 231 (443) \\
$4$ balls & 2.67 (1.95) & 8.01 (4.53) & 24.5 (19.0) & 121 (169) \\
$5$ balls & {\bf 2.66 (1.73)} & {\bf 6.98 (4.25)} & {\bf 23.3 (14.8)} & {\bf 104 (91)} \\
$6$ balls & 8.68 (6.62) & 29.1 (15.8) & 83.0 (66.7) & 286 (407) \\
$7$ balls & 10.1 (5.34) & 39.4 (15.2) & 108 (74.5) & 294 (226) \\
\bottomrule
\end{tabular}
\end{center}
\end{table}
